Direction-Aware Offline-to-Online Learning in Linear Contextual Bandits

Many bandit systems are deployed with offline historical data, such as past logs from earlier policies. Using these data can reduce early online exploration when they remain informative for the online problem. When the offline and online environments differ, such data can be biased for the online problem. For linear (contextual) bandits, this bias is directional: offline data may be informative in some feature directions and misleading in others. However, prior work typically controls this gap through a known Euclidean bound on the model parameters, which we prove is too coarse: even with the offline parameter known, bias in a single unknown direction can force dimension-dependent regret. To address this challenge, we introduce a directional bias certificate $(M_{\mathrm{bias}},\rho)$ that measures the offline-to-online gap through an $M_{\mathrm{bias}}$-induced norm and assigns different bias budgets to different directions. Building on this certificate, we propose \emph{Ellipsoidal-MINUCB}, which augments the online learning with an offline-pooled branch that safely exploits historical data. When the certificate is known, we show that the algorithm matches the standard SupLinUCB rate in the worst case and improves when offline coverage aligns with low-bias directions. When the certificate is unknown, we estimate it adaptively from offline and accumulated online data and establish a corresponding regret guarantee. Numerical experiments support the theory and show gains in aligned regimes.

==> sections/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

A key insight of this paper is that biased offline data in linear contextual bandits are not useful
as a single warm start. They are useful only along directions that are both well covered offline and
stable under offline-to-online shift. The directional certificate $(M_{\mathrm{shift}},\rho)$ makes
this criterion for offline quality explicit, and Ellipsoidal-MINUCB turns it into a safe
algorithmic rule: exploit pooled geometry where transfer is credible, and fall back to the classical
online branch elsewhere.

The analysis preserves this safety story at the regret level: the high-probability bound is the
\emph{minimum} of a standard SupLinUCB-type online term and a geometry-dependent pooled term. Poor
transfer therefore cannot erase the explicit $\widetilde{O}(\sqrt{dT})$ fallback. The main
limitation is that the certificate is side information, and the pooled term may depend on the online
path. Natural next steps are data-driven certificates with graceful degradation under approximate
transfer, and extensions beyond linear models.

%\paragraph{Broader impact.}
%Biased offline logs appear in advertising, pricing, recommendation, and other sequential decision
%systems. Safer reuse of such data can reduce online exploration cost. The corresponding risk is that
%an over-trusted certificate may entrench historical bias by declaring unstable directions safe.
%Conservative certificates and small online calibration sets are therefore important in high-stakes
%or fairness-sensitive deployments.


==> sections/experiments.tex <==
\section{Experiments}
\label{sec:experiments}
\FloatBarrier

We evaluate Ellipsoidal-MINUCB in synthetic linear contextual bandits with
$K{=}5$ arms, $d{=}5$ features, horizon $T{=}20000$, sub-Gaussian reward noise~$\sigma{=}0.1$, and
$n_{\mathrm{off}}{=}2000$ offline points.
Arms' feature vectors are drawn from a Gaussian, then normalized to the Euclidean unit ball (the same
protocol as in the released implementation).
We use ridge regularization $\lambda_{\mathrm{reg}}{=}1$ and confidence and certificate parameters
$\delta{=}0.01$, $\gamma_{\mathrm{cert}}{=}1.04$, and we average $5$ random seeds in each run.

Figure~\ref{fig:exp-main} reports cumulative regret in three \emph{matched} misspecification regimes.
In all three, the coordinates not shown below are set to~$1$, and the shift is concentrated on a pair of
entries of $\theta_*$ and~$\theta^\dagger$:
\emph{(i)}~$(\theta_{*,1},\theta^\dagger_2)=(1.1,1.1)$;
\emph{(ii)}~$(2,2)$;
\emph{(iii)}~$(10,10)$ (the first example is a mild, symmetric perturbation; the last is a large
first-coordinate mass scale).
The figure compares a standard SupLinUCB baseline, Ellipsoidal-MINUCB, a warm-started SupLinUCB, and a
non-adaptive policy that uses only the offline estimate (no online parameter update).
Pooled and warm-start policies improve most clearly in the middle regime, while the largest separation
makes the shift cost dominate and re-aligns behavior with the safe online objective.

\begin{figure}[H]
  \centering
  \includegraphics[width=\linewidth]{exp00_main/regret_curves.pdf}
  \caption{Main synthetic study: mean cumulative regret with variability bands across
  seeds. The three panels use increasing shift mass on a shared two-coordinate family as described in
  the main text; algorithms are the SupLinUCB baseline, Ellipsoidal-MINUCB, a warm start, and an
  offline-only baseline.}
  \label{fig:exp-main}
\end{figure}

\paragraph{Additional experiments.}
Appendix~\ref{app:more-experiments} reports three additional experiments: randomized shift generation that
trades a multiplicative component against an additive offset; fixed $\theta_*$ with varying alignment of
the offline mean; and \emph{offline} covariate support held strictly inside the \emph{online} support, so
that the offline design matrix is rank-deficient in some directions when the two parameters align.
\FloatBarrier


==> sections/introduction.tex <==
\section{Introduction}
\label{sec:intro}

Many bandit deployments start with historical logs, A/B traffic, or related populations. Exploiting
this data could reduce cold-start exploration, but the offline model is often trained under a
different decision policy, population, or feature distribution than the live system. The resulting
\emph{misspecification} is not a small nuisance: treating an offline point estimate as if it were the
online truth can be arbitrarily misleading once deployment begins.

We focus on \emph{linear contextual bandits}, where arms share a feature map in $\R^d$ and rewards
are linear in a shared parameter. This shared-parameter structure changes the question: offline
usefulness is not a list of arm-specific biases, but a problem of \emph{which directions} in feature
space remain informative for online play.

Usefulness is intrinsically \emph{directional}. Offline-to-online gap is generally anisotropic: a
single Euclidean radius treats all feature directions equally, which can be simultaneously too loose
in stable directions and too aggressive where shift is large. Analyses of biased prior data at the
arm level (e.g., MIN-UCB) and of mismatch through scalar summaries in simpler action models
\citep{cheung2024} do not directly lift to a global linear feature map without an explicit geometric
interface. Prior work on leveraging offline design in linear bandits often studies \emph{coverage}
under the idealization that the offline and online parameters coincide \citep{vijayan2025oope}. We
target the mixed regime: offline samples may be \emph{rich in some directions and misleading in
others} while the user can supply a matrix-shaped description of which directions are plausible
under shift.

We take as side information a shift certificate
$\|\theta_*-\theta^\dagger\|_{M_{\mathrm{shift}}}\le \rho$ together with a standard offline ridge
estimate and its design matrix. This yields a confidence description for the online target that
\emph{separates} statistical error (through the offline Gram) from shift (through
$(M_{\mathrm{shift}},\rho)$) along each queried feature direction. The algorithmic object is
\emph{Ellipsoidal-MINUCB}, built on the SupLinUCB shell \citep{chu2011}: a standard online
confidence branch and a pooled branch that mixes offline and online Gram information; UCB/LCB
scores are merged so that the pooled information is used only when it is tighter. The end result is
a per-round \emph{minimum} of online and offline-informed optimism, hence a retained
$\widetilde{O}(\sqrt{dT})$ online fallback (SupLinUCB type) is explicit in the analysis.
Our end goal is not a new generic SupLinUCB-style master rule in isolation, but a modeling and
decision interface for \emph{directional} misspecification: the certificate and offline design
specify which directions are simultaneously well measured and safe to pool, while a standard
online confidence branch remains a round-by-round fallback; Section~\ref{sec:theory} makes the
ensuing \emph{min}-type regret bound explicit.
Good offline data combine (i) enough effective \emph{sample size} to shrink offline regression error,
(ii) a \emph{coverage} shape in which the directions queried online are actually measured, and
(iii) a conservative but valid \emph{shift} envelope; increasing data alone does not fix a
misspecified shift model when the online-requested directions are expensive under the certificate.

In practice, a valid~$(M_{\mathrm{shift}},\rho)$ may be unavailable a priori; we therefore also
develop a \emph{data-driven} certificate updated at finitely many epoch boundaries, with
statements, routing formulas, and regret guarantees in
Section~\ref{sec:epoch-wise-ell-minucb} and Appendices~\ref{app:epoch-dd-details} and~\ref{app:epoch-learned-proofs}.

\medskip
\noindent\textbf{Contributions.}\par
\smallskip
\begin{itemize}
\item \textbf{Directional certificate.}
      We use the directional certificate $(M_{\mathrm{shift}},\rho)$ as a natural geometric interface
      for offline quality: it encodes which directions are transferable and yields a
      geometry-aware confidence description rather than a scalar trust radius.
\item \textbf{Algorithm Design.}
      We introduce \emph{Ellipsoidal-MINUCB}: a two-branch optimistic procedure with an always-safe online branch and an
      offline-informed pooled branch; min/max aggregation ensures the pooled branch only acts when
      it is tighter, while the online branch remains a round-by-round fallback.
      Section~\ref{sec:algorithm} also records diagnostic quantities for when pooling helps in practice.
\item \textbf{Data-driven certificates.}
      When a valid~$(M_{\mathrm{shift}},\rho)$ is not available a priori, we construct a matrix--radius
      pair at finitely many epoch boundaries from the offline design matrix and the online ridge
      state, using the parallel sum of the two regularized Gram matrices so the center gap and
      shift map are measured in a \emph{shared} norm geometry. The min/max layer policy of
      Section~\ref{sec:algorithm} is unchanged except for re-parameterized pooled radii and routings
      (Section~\ref{sec:epoch-wise-ell-minucb}).
\item \textbf{Theory.}
      We prove a high-probability regret guarantee given by the minimum of the standard SupLinUCB
      fallback \citep{chu2011} and a geometry-dependent pooled term, and we show how directional
      usefulness appears through a pooled-width decomposition.
      Under an alignment condition between offline precision and shift, the pooled analysis yields a
      clean effective-dimension regime. We also give a separation for purely Euclidean (scalar) shift
      summaries (Appendix~\ref{app:isotropic-too-coarse}).
      For the epoch-wise data-driven construction in Section~\ref{sec:epoch-wise-ell-minucb}, we
      establish a high-probability regret bound over the epoch boundaries at
      which the certificate is updated (proofs in Appendix~\ref{app:epoch-learned-proofs}).
\end{itemize}

\smallskip
\noindent\textit{Organization.}
Sections~\ref{sec:setup}--\ref{sec:experiments} present the model, Ellipsoidal-MINUCB, main results,
data-driven certificates, and experiments; related work and the conclusion follow.
The appendix contains proofs and supplements, including isotropic and diagonal specializations
(Appendices~\ref{app:isotropic-too-coarse} and~\ref{app:diagonal-specialization}), data-driven
certificate details and proofs (Appendices~\ref{app:epoch-dd-details} and~\ref{app:epoch-learned-proofs}),
notation (Appendix~\ref{app:notation}), and additional experiments (Appendix~\ref{app:more-experiments}).


==> sections/method.tex <==
\section{Problem Setup}
\label{sec:setup}

We specify the online bandit model, offline regression data, and a shift certificate, then record an
offline confidence region for $\theta_*$ used in Section~\ref{sec:algorithm}.

Let $\cF_{t-1}$ be the $\sigma$-algebra generated by $(x_{s,\cdot},a_s,r_s)_{s<t}$ and the current
contexts $\{x_{t,a}\}_{a\in[K]}$. We consider a stochastic linear contextual bandit over horizon $T$.

\begin{assumption}[Linear reward with bounded features]
\label{asm:linear}
At each round $t\in[T]$, the learner observes a finite action set
$\{x_{t,a}\}_{a \in [K]} \subset \R^d$ with $\|x_{t,a}\|_2 \le 1$, selects $a_t$, and receives
$r_t = x_{t,a_t}^{\top}\theta_* + \eta_t \in [0,1]$, where $\theta_* \in \R^d$ is unknown with
$\|\theta_*\|_2 \le S$. The action set at round $t$ is revealed before the reward is observed, so
$x_{t,a_t}$ and the SupLinUCB layer assignment (Section~\ref{sec:algorithm}) are
$\cF_{t-1}$-measurable.
\end{assumption}

\begin{assumption}[Conditionally sub-Gaussian online noise]
\label{asm:subg}
$\E[\eta_t \mid \cF_{t-1}] = 0$ and $\eta_t$ is conditionally $\sigma$-sub-Gaussian given
$\cF_{t-1}$. Bounded features together with $\|\theta_*\|_2 \le S$ imply $\eta_t$ is bounded, so the
sub-Gaussian tail model is standard (constants may be absorbed into $\sigma$).
\end{assumption}

The cumulative regret is
\[
R_T := \sum_{t=1}^T \left( \max_{a \in [K]} x_{t,a}^{\top}\theta_* - x_{t,a_t}^{\top}\theta_* \right).
\]

Before the online phase, the learner observes an offline regression sample
$D_{\mathrm{off}} = \{(z_i,y_i)\}_{i=1}^{n_{\mathrm{off}}}$. The difficulty is that the offline
parameter $\theta^\dagger$ need not equal the online parameter $\theta_*$.

\begin{assumption}[Offline regression sample]
\label{asm:offline}
$y_i = z_i^{\top}\theta^\dagger + \xi_i$ with $\|z_i\|_2\le 1$, $\|\theta^\dagger\|_2\le S$, and
$\E[\xi_i\mid z_i]=0$. The offline covariates $\{z_i\}$ are non-adaptive (fixed before the online
phase), and $\xi_i$ is conditionally $\sigma$-sub-Gaussian given $z_i$.
\end{assumption}

\begin{definition}[Directional shift certificate]
\label{def:certificate}
A pair $(M_{\mathrm{shift}},\rho)$ is a valid shift certificate if $M_{\mathrm{shift}} \succ 0$ is
known and
\[
\|\theta_*-\theta^\dagger\|_{M_{\mathrm{shift}}} \le \rho.
\]
Equivalently, every direction $x \in \R^d$ satisfies
\[
|x^{\top}(\theta_*-\theta^\dagger)| \le \rho \|x\|_{M_{\mathrm{shift}}^{-1}}.
\]
Throughout, we treat $(M_{\mathrm{shift}},\rho)$ as fixed side information. When it is estimated
before deployment, guarantees hold conditional on validity.
\end{definition}

\paragraph{Interpretation of the certificate.}
In linear contextual bandits, rewards depend on actions only through features, so the natural
object to control is parameter error \emph{along the directions} that enter UCB/LCB scores.
A valid $(M_{\mathrm{shift}},\rho)$ is side information that encodes this anisotropy: it implies
per-direction bounds with penalties $\rho\|x\|_{M_{\mathrm{shift}}^{-1}}$ matching the linear
optimistic template, and it is not identified from bandit feedback alone without additional
structure.
By contrast, a Euclidean certificate $\norm{\theta_*-\theta^\dagger}_2 \le \rho$ controls only the
\emph{magnitude} of the shift and can hide whether misspecification lies along a regret-relevant
direction.
Appendix~\ref{app:isotropic-too-coarse} gives a finite-action Bernoulli specialization in which
three instances share the same offline parameter and offline data law and satisfy the same scalar
radius; in one case a fixed action is optimal throughout, while in a paired hard case the learner
must identify the sign of a hidden shift and every policy suffers regret of order
$\rho^2T/\rho_0$ on one of the two instances.

To use this side information algorithmically, we combine it with the standard offline ridge
estimate. The offline sample yields a confidence ellipsoid around $\theta^\dagger$. Together with the
shift certificate, the next proposition fuses the two into a single confidence region for
$\theta_*$.

The offline sample induces the usual ridge objects
\[
G_{\mathrm{off}} := I + \sum_{i=1}^{n_{\mathrm{off}}} z_i z_i^{\top},
\qquad
\hat\theta_{\mathrm{off}} := G_{\mathrm{off}}^{-1} \sum_{i=1}^{n_{\mathrm{off}}} z_i y_i.
\]
Here $G_{\mathrm{off}}$ records offline coverage, while $\hat\theta_{\mathrm{off}}$ estimates the
offline parameter $\theta^\dagger$. A standard ridge concentration inequality controls
$\hat\theta_{\mathrm{off}}-\theta^\dagger$ in the $G_{\mathrm{off}}$ metric; the certificate then
lifts this offline ellipsoid to a confidence region for $\theta_*$.

\begin{proposition}[Offline-to-online confidence region]
\label{prop:offline-region}
For
\[
\beta_{\mathrm{off}}(\delta) :=
\sigma \sqrt{2 \log \frac{\det(G_{\mathrm{off}})^{1/2}}{\delta}}
+ S,
\]
with probability at least $1-\delta$,
\[
\theta_* \in
\left\{
\hat\theta_{\mathrm{off}} + u + v :
\|u\|_{G_{\mathrm{off}}} \le \beta_{\mathrm{off}}(\delta),
\ \|v\|_{M_{\mathrm{shift}}} \le \rho
\right\}
=:
\cC_{\mathrm{off}}.
\]
Consequently, the support function of this region is
\[
\sup_{\theta \in \cC_{\mathrm{off}}} x^{\top}\theta
=
x^{\top}\hat\theta_{\mathrm{off}}
+ \beta_{\mathrm{off}}(\delta)\|x\|_{G_{\mathrm{off}}^{-1}}
+ \rho\|x\|_{M_{\mathrm{shift}}^{-1}}.
\]
\end{proposition}

Proposition~\ref{prop:offline-region} writes $\theta_*$ as lying in a Minkowski sum of two ellipsoids:
statistical uncertainty around $\hat\theta_{\mathrm{off}}$ (radius $\beta_{\mathrm{off}}(\delta)$ in the
$G_{\mathrm{off}}^{-1}$ metric) and shift uncertainty (radius $\rho$ in the $M_{\mathrm{shift}}^{-1}$
metric). This is the offline building block of the pooled branch in
Section~\ref{sec:algorithm}: the displayed support function is the resulting \emph{directional}
confidence radius for $x^\top\theta_*$. In short, \emph{bias} enters through $\rho$ and
$M_{\mathrm{shift}}$. \emph{Sample size} and \emph{diversity} enter through $G_{\mathrm{off}}$ and
$\beta_{\mathrm{off}}(\delta)$. Increasing $n_{\mathrm{off}}$ alone does not remove the shift term
under a fixed certificate. The cases
$M_{\mathrm{shift}}=I$, diagonal $M_{\mathrm{shift}}$, or $M_{\mathrm{shift}}$ nearly singular on a
subspace correspond respectively to isotropic shift, per-coordinate budgets, and shift confined to a few
directions.

\section{Ellipsoidal-MINUCB}
\label{sec:algorithm}

So far, $\theta_*$ is described only through the offline-informed region above. Online play requires
layerwise scores that update with streaming data. The next paragraphs define those scores.
Algorithm~\ref{alg:ellipsoidal-minucb} records the SupLinUCB elimination loop.

\paragraph{Online branch.}
For each layer $\ell$, let $A_{t,\ell}$ be the layerwise online Gram matrix,
$V_{t,\ell} := I + A_{t,\ell}$, and
\[
\hat\theta^{\mathrm{on}}_{t,\ell} := V_{t,\ell}^{-1} b_{t,\ell},
\qquad
b_{t,\ell} := \sum_{s \in \cH_{t,\ell}} x_{s,a_s} r_s.
\]
The online UCB (upper confidence bound) score is
\[
U^{\mathrm{on}}_{t,\ell}(a)
=
x_{t,a}^{\top}\hat\theta^{\mathrm{on}}_{t,\ell}
+ \beta^{\mathrm{on}}_{t,\ell}\|x_{t,a}\|_{V_{t,\ell}^{-1}},
\]
with the corresponding online LCB (lower confidence bound) $L^{\mathrm{on}}_{t,\ell}(a)$, where
\[
\beta^{\mathrm{on}}_{t,\ell}
:=
\sigma \sqrt{2 \log \frac{\det(V_{t,\ell})^{1/2}}{\delta^{\mathrm{on}}_{t,\ell}}}
+ S
\]
is the layerwise ridge confidence radius for budget $\delta^{\mathrm{on}}_{t,\ell}$.

\paragraph{Pooled branch.}
The offline-informed estimator is
\[
\hat\theta^{\mathrm{pool}}_{t,\ell}
:=
(A_{t,\ell}+G_{\mathrm{off}})^{-1}
\bigl(b_{t,\ell} + G_{\mathrm{off}}\hat\theta_{\mathrm{off}}\bigr).
\]
The confidence interval radius is
\[
\mathrm{rad}^{\mathrm{pool}}_{t,\ell}(x)
:=
\bigl(\gamma_{t,\ell}+\beta_{\mathrm{off}}\bigr)\|x\|_{(A_{t,\ell}+G_{\mathrm{off}})^{-1}}
+ \rho \,\psi_{t,\ell}(x),
\]
where
\[
\psi_{t,\ell}(x)
:=
\left\|
M_{\mathrm{shift}}^{-1/2}
G_{\mathrm{off}}(A_{t,\ell}+G_{\mathrm{off}})^{-1}x
\right\|_2.
\]
The pooled martingale radius is
\[
\gamma_{t,\ell}
:=
\sigma \sqrt{2 \log \frac{\det(V_{t,\ell})^{1/2}}{\delta^{\mathrm{pool}}_{t,\ell}}}
+ S.
\]
The pooled UCB is
\[
U^{\mathrm{pool}}_{t,\ell}(a)
=
x_{t,a}^{\top}\hat\theta^{\mathrm{pool}}_{t,\ell}
+ \mathrm{rad}^{\mathrm{pool}}_{t,\ell}(x_{t,a}),
\]
with the corresponding pooled LCB $L^{\mathrm{pool}}_{t,\ell}(a)$ defined symmetrically.

\paragraph{Interpretation of the pooled confidence radius.}
Pooling replaces $\|x\|_{V_{t,\ell}^{-1}}$ by $\|x\|_{(A_{t,\ell}+G_{\mathrm{off}})^{-1}}$ when
offline mass adds precision along $x$. The term $\rho\,\psi_{t,\ell}(x)$ is the shift premium routed
through $G_{\mathrm{off}}(A_{t,\ell}+G_{\mathrm{off}})^{-1}$ and $M_{\mathrm{shift}}$. The same
display splits the width into online fluctuation $\gamma_{t,\ell}$, offline ridge slack
$\beta_{\mathrm{off}}$, and mismatch, all in the pooled metric: the linear analogue of a
variance--bias decomposition. Help on a direction requires the first two pieces to dominate the third.

\paragraph{Branch aggregation.}
The final aggregated UCB and LCB are
\[
U^{\min}_{t,\ell}(a)
:=
\min\{U^{\mathrm{on}}_{t,\ell}(a),U^{\mathrm{pool}}_{t,\ell}(a)\},
\qquad
L^{\max}_{t,\ell}(a)
:=
\max\{L^{\mathrm{on}}_{t,\ell}(a),L^{\mathrm{pool}}_{t,\ell}(a)\}.
\]
This design makes the safety mechanism explicit: the pooled branch can only help if it is tighter,
and the online branch remains available term by term when the certificate is weak or the queried
direction is poorly covered offline.

\paragraph{Directional helpfulness of offline data.}
Set
\[
\mathrm{rad}^{\mathrm{on}}_{t,\ell}(x)
:=
\beta^{\mathrm{on}}_{t,\ell}\|x\|_{V_{t,\ell}^{-1}},
\qquad
\Delta_{t,\ell}(x)
:=
\mathrm{rad}^{\mathrm{on}}_{t,\ell}(x)
-
\mathrm{rad}^{\mathrm{pool}}_{t,\ell}(x),
\]
and the offline summary
\[
h_{\mathrm{off}}(x)
:=
\beta_{\mathrm{off}}\|x\|_{G_{\mathrm{off}}^{-1}}
+
\rho\|x\|_{M_{\mathrm{shift}}^{-1}}.
\]
Positive $\Delta_{t,\ell}(x)$ means the pooled interval is narrower than the online one along $x$;
small $h_{\mathrm{off}}(x)$ marks directions that are both well covered offline and cheap under shift.
Nesting and screening conditions are in Appendix~\ref{app:directional-helpfulness}
(Proposition~\ref{prop:helpfulness} and Corollary~\ref{cor:helpfulness-screen}).

Let
\[
w_{t,\ell}(a) := U^{\min}_{t,\ell}(a)-L^{\max}_{t,\ell}(a)
\]
denote the aggregated interval width. Algorithm~\ref{alg:ellipsoidal-minucb} states the layerwise
SupLinUCB shell with explicit online and pooled confidence schedules.

\begin{algorithm}[t]
\caption{Ellipsoidal-MINUCB}
\label{alg:ellipsoidal-minucb}
\begin{algorithmic}[1]
\Require Offline data $D_{\mathrm{off}}$, certificate $(M_{\mathrm{shift}},\rho)$, horizon $T$,
online confidence schedule
$\{\delta^{\mathrm{on}}_{t,\ell}\}_{t \le T,\ell \le \lceil \log_2 T \rceil}$, and pooled
confidence schedule $\{\delta^{\mathrm{pool}}_{t,\ell}\}_{t \le T,\ell \le \lceil \log_2 T \rceil}$
\State Compute $G_{\mathrm{off}}$, $\hat\theta_{\mathrm{off}}$, and $\beta_{\mathrm{off}}$ from
$D_{\mathrm{off}}$
\State $L \gets \lceil \log_2 T \rceil$
\State Initialize $\cH_{1,\ell} \gets \varnothing$ for all $\ell = 0,1,\dots,L$
\For{$t = 1,2,\dots,T$}
    \State Set $\cH_{t+1,\ell} \gets \cH_{t,\ell}$ for every $\ell = 0,1,\dots,L$
    \State Observe the action set $\{x_{t,a}\}_{a \in [K]}$
    \State $\cA_{t,0} \gets [K]$
    \For{$\ell = 0,1,\dots,L$}
        \State Build $A_{t,\ell}$, $V_{t,\ell}$, $b_{t,\ell}$, the online UCB/LCB and pooled UCB/LCB
        from $\cH_{t,\ell}$
        \For{each $a \in \cA_{t,\ell}$}
            \State Compute aggregated UCB $U^{\min}_{t,\ell}(a)$, aggregated LCB $L^{\max}_{t,\ell}(a)$, and $w_{t,\ell}(a)$
        \EndFor
        \If{$\ell = L$}
            \State Play $a_t \in \argmax_{a \in \cA_{t,\ell}} U^{\min}_{t,\ell}(a)$
            \State Observe reward $r_t$ and append $(x_{t,a_t},r_t)$ to $\cH_{t+1,\ell}$
            \State Record $\ell_t \gets \ell$ and break the layer loop
        \ElsIf{$\max_{a \in \cA_{t,\ell}} w_{t,\ell}(a) > 2^{-\ell}$}
            \State Play
            $a_t \in \argmax_{a \in \cA_{t,\ell}: w_{t,\ell}(a) > 2^{-\ell}} U^{\min}_{t,\ell}(a)$
            \State Observe reward $r_t$ and append $(x_{t,a_t},r_t)$ to $\cH_{t+1,\ell}$
            \State Record $\ell_t \gets \ell$ and break the layer loop
        \Else
            \State $m_{t,\ell} \gets \max_{a \in \cA_{t,\ell}} L^{\max}_{t,\ell}(a)$
            \State
            $\cA_{t,\ell+1}
            \gets
            \{a \in \cA_{t,\ell} : U^{\min}_{t,\ell}(a) \ge m_{t,\ell}\}$
        \EndIf
    \EndFor
\EndFor
\end{algorithmic}
\end{algorithm}

\section{Main Results}
\label{sec:theory}

The next theorem states our main high-probability regret bound; corollaries and structural comparisons
follow in the same section.

\begin{theorem}[High-probability guarantee]
\label{thm:main}
Run Ellipsoidal-MINUCB with confidence budgets
$\delta_{\mathrm{off}},\delta_{\mathrm{on}},
\{\delta_{t,\ell}^{\mathrm{on}}\},\{\delta_{t,\ell}^{\mathrm{pool}}\}$ satisfying
\[
\sum_{t=1}^T\sum_{\ell=0}^{\lceil\log_2 T\rceil}\delta_{t,\ell}^{\mathrm{on}}
\le \delta_{\mathrm{on}},
\qquad
\delta_{\mathrm{off}}+\delta_{\mathrm{on}}
+\sum_{t=1}^T\sum_{\ell=0}^{\lceil\log_2 T\rceil}\delta_{t,\ell}^{\mathrm{pool}}
\le T^{-2}.
\]
Then, with probability at least $1-T^{-2}$,
\[
R_T
\le
\min\left\{
C_{\mathrm{SL}}\sqrt{Td\,L_T^3},
\;
8\sum_{\ell=0}^{\lceil\log_2 T\rceil}
\bigl(\beta_{\mathrm{off}}+\gamma_\ell^{\mathrm{fin}}\bigr)
\sqrt{2|Q_\ell|\,\Lambda_\ell}
+ 8\rho\,\widetilde\Psi_T
\right\},
\]
where
\[
Q_\ell
:=
\{t\in[T]:\ell_t=\ell\},
\qquad
A_\ell^{\mathrm{fin}}
:=
\sum_{t\in Q_\ell}x_{t,a_t}x_{t,a_t}^{\top},
\]
\[
V_\ell^{\mathrm{fin}}
:=
I+A_\ell^{\mathrm{fin}},
\qquad
\Lambda_\ell
:=
\log \frac{\det(A_\ell^{\mathrm{fin}} + G_{\mathrm{off}})}{\det(G_{\mathrm{off}})},
\qquad
\widetilde\Lambda_T
:=
\sum_{\ell=0}^{\lceil\log_2 T\rceil}\Lambda_\ell,
\]
\[
\widetilde\Psi_T
:=
\sum_{t=1}^T \psi_{t,\ell_t}(x_{t,a_t}),
\qquad
\delta_{\ell,\min}^{\mathrm{pool}}
:=
\min_{t\le T}\delta_{t,\ell}^{\mathrm{pool}},
\]
\[
\gamma_\ell^{\mathrm{fin}}
:=
\sigma \sqrt{2 \log \frac{\det(V_\ell^{\mathrm{fin}})^{1/2}}{\delta_{\ell,\min}^{\mathrm{pool}}}}
+ S,
\qquad
\beta_{\mathrm{off}} := \beta_{\mathrm{off}}(\delta_{\mathrm{off}}),
\qquad
L_T := \log\!\bigl(2KT\log T/\delta_{\mathrm{on}}\bigr).
\]
In particular,
\[
R_T
\le
\min\left\{
C_{\mathrm{SL}}\sqrt{Td\,L_T^3},
\;
8\beta_\star\sqrt{2T\,\widetilde\Lambda_T}
+ 8\rho\,\widetilde\Psi_T
\right\},
\]
where
\[
\delta_{\min}^{\mathrm{pool}}
:=
\min_{t,\ell}\delta_{t,\ell}^{\mathrm{pool}},
\qquad
\beta_\star
:=
\beta_{\mathrm{off}}
+
\sigma \sqrt{d\log(1+T)+2\log(1/\delta_{\min}^{\mathrm{pool}})}
+ S.
\]
\end{theorem}

The first term is the ordinary SupLinUCB fallback. The second is the pooled term, whose gain is
tracked by $\widetilde\Lambda_T$ and whose shift cost is tracked by $\widetilde\Psi_T$ along the
realized trajectory. Neither pooled expression need dominate uniformly on every instance or every
prefix, so the clearest gains often appear at intermediate horizons.

The only part of the pooled bound that is not yet expressed through log-determinant geometry is the
routed shift term $\widetilde\Psi_T$. The next proposition controls it under an alignment condition
between offline precision and shift.

\begin{proposition}[Computable pooled regime]
\label{prop:pooled-geometry}
If
\[
G_{\mathrm{off}} M_{\mathrm{shift}}^{-1} G_{\mathrm{off}}
\preceq
c_{\mathrm{shift}}\, G_{\mathrm{off}}
\]
for some $c_{\mathrm{shift}} \ge 0$, then
\[
\widetilde\Psi_T \le \sqrt{2 c_{\mathrm{shift}} T\,\widetilde\Lambda_T},
\]
and the pooled branch in Theorem~\ref{thm:main} simplifies to
\[
R_T \le
8\beta_\star\sqrt{2T\,\widetilde\Lambda_T}
+ 8\rho\sqrt{2 c_{\mathrm{shift}} T\,\widetilde\Lambda_T}
= O(\sqrt{T\,\widetilde\Lambda_T}).
\]
\end{proposition}

\begin{corollary}[Effective-dimension improvement regime]
\label{cor:effective-dim}
Assume the condition of Proposition~\ref{prop:pooled-geometry}. If, in addition,
\[
\widetilde\Lambda_T \le d_{\mathrm{eff}}\log(1+T)
\]
for some $d_{\mathrm{eff}}\in[0,d]$, then on the event of Theorem~\ref{thm:main},
\[
R_T
\le
8\bigl(\beta_\star+\rho\sqrt{c_{\mathrm{shift}}}\bigr)
\sqrt{2T\,d_{\mathrm{eff}}\log(1+T)}.
\]
\end{corollary}

The condition in Proposition~\ref{prop:pooled-geometry} says that directions with strong offline
precision do not simultaneously carry arbitrarily large shift uncertainty. Under it,
Corollary~\ref{cor:effective-dim} replaces the ambient dimension by an effective dimension scale
determined by the realized offline-supported trajectory. If the certificate is conservative but
valid, the pooled term merely widens and the method falls back more often to the online branch. If
the radius is undersized so that the true shift is excluded, then the pooled branch should be read
as a heuristic warm start rather than as part of the theorem's guarantee.

\begin{theorem}[Lower bound for isotropic certificates]
\label{thm:lower}
Assume $K\ge d-1$ and $S\ge 1$. There exists a universal constant $c>0$ such that, for all
$d\ge 9$ and $T\ge d^2$, even in the stronger oracle model where the learner
is given the offline reference parameter $\theta^\dagger$ in advance, the worst-case regret over the isotropic subclass
$\|\theta_*-\theta^\dagger\|_2 \le \rho$ is at least of order
\[
c\,\min\{\rho T,\sqrt{dT}\}.
\]
\end{theorem}

This lower bound records the limitation of scalar certificates: they cannot by themselves capture
the directional structure that drives transfer in the linear setting. When actions are orthonormal and $G_{\mathrm{off}}$ and $M_{\mathrm{shift}}$ are diagonal in a shared basis, the pooled UCB decouples into an arm-wise pseudo-count and bias-budget form parallel in structure to MIN-UCB \citep{cheung2024} (Appendix~\ref{app:diagonal-specialization} gives the specialization and an activation corollary); this is a structural diagnostic and does not identify the policies. Proofs of the results in this section are deferred to the appendix.

\section{Data-Driven Directional Shift Certificates}
\label{sec:epoch-wise-ell-minucb}

When a valid fixed certificate~$(M_{\mathrm{shift}},\rho)$ is unavailable, we construct a
matrix--radius pair~$(\widehat M_k,\widehat\rho_k)$ at finitely many epoch boundaries from the offline
design~$G_{\mathrm{off}}$ and the online ridge state accumulated to each refresh, and keep it
constant between updates.
The min/max layer policy of Section~\ref{sec:algorithm} is unchanged: only the pooled radii and shift
routing are re-parameterized.
Routing formulas, validity of the learned map, a doubling-epoch schedule, and the statement and proof
of the corresponding certificate event are in
Appendices~\ref{app:epoch-dd-details} and~\ref{app:epoch-learned-proofs}.
The construction and per-epoch definitions are spelled out next, and
Algorithm~\ref{alg:epoch-ell-minucb} records the update loop.

\paragraph{Epoch construction.}
Fix
\(
1=\tau_1<\cdots<\tau_{K_{\mathrm{ep}}}\le T
\)
with
\(
\tau_{K_{\mathrm{ep}}+1}:=T+1
\).
(Equally spaced, doubling, or other rules can be used; $\tau_1=1$ so the first certificate may depend
only on~$D_{\mathrm{off}}$ plus any pre-deployment information.)
For each~$k$, before round~$\tau_k$, from past \emph{online} rounds only, define
\[
G_k^{\mathrm{on}}
:=
I+\sum_{s<\tau_k}x_{s,a_s}x_{s,a_s}^{\top},
\qquad
\hat\theta_k^{\mathrm{on}}
:=
(G_k^{\mathrm{on}})^{-1}\sum_{s<\tau_k}x_{s,a_s}r_s.
\]
The epoch certificate sets~$\widehat M_k$ to the \emph{parallel sum} of~$G_k^{\mathrm{on}}$ and~$G_{\mathrm{off}}$,
\(
\widehat M_k
:=\bigl((G_k^{\mathrm{on}})^{-1}+G_{\mathrm{off}}^{-1}\bigr)^{-1}
\),
and the radius
\[
\widehat\rho_k
:=
\|\hat\theta_k^{\mathrm{on}}-\hat\theta_{\mathrm{off}}\|_{\widehat M_k}
+
\beta_k^{\mathrm{on}}(\delta_k)
+
\beta_{\mathrm{off}}(\delta_{\mathrm{off}}),
\]
where $\beta_k^{\mathrm{on}}(\delta_k)$ is any valid ridge self-normalized bound for~$\theta_*$ in
the $G_k^{\mathrm{on}}$-norm (evaluated on data up to, but not including, round~$\tau_k$).
Rounds $t\in\{\tau_k,\ldots,\tau_{k+1}-1\}$ use the min/max layer shell of
Section~\ref{sec:algorithm}, replacing the fixed-certificate map $\psi_{t,\ell}$ by
$\widehat\psi_{k,t,\ell}$ in \eqref{eq:epoch-psi} and $\mathrm{rad}^{\mathrm{pool}}_{t,\ell}$ by
$\widehat{\mathrm{rad}}^{\mathrm{pool,ep}}_{t,\ell}$ in \eqref{eq:epoch-pool-rad} of
Appendix~\ref{app:epoch-dd-details}. The min/max structure is unchanged, so the online branch remains
a safe fallback when $\widehat\rho_k$ is large.
Under the usual ridge events and a union bound on an appropriate schedule
for $\{\delta_k\}_{k=1}^{K_{\mathrm{ep}}}$ (with
$\delta_{\mathrm{off}}+\sum_k\delta_k\le\delta_{\mathrm{cert}}$), this~$\widehat M_k$ yields
$\|\theta_*-\theta^\dagger\|_{\widehat M_k}\le\widehat\rho_k$ for all epochs on an event of
probability at least $1-\delta_{\mathrm{cert}}$; see
Theorem~\ref{thm:epoch-parallel-cert-valid} in Appendix~\ref{app:epoch-dd-details}.

\begin{algorithm}[t]
\caption{Data-Driven Directional Ellipsoidal-MINUCB}
\label{alg:epoch-ell-minucb}
\begin{algorithmic}[1]
\Require $D_{\mathrm{off}}$, $T$, prespecified
\(
1{=}\tau_1{<}\cdots{<}\tau_{K_{\mathrm{ep}}}{\le}T
\)
and
\(
\tau_{K_{\mathrm{ep}}+1}{=}T{+}1
\);
confidence schedules
$\{\delta_{t,\ell}^{\mathrm{on}}\}$,
$\{\delta_{t,\ell}^{\mathrm{pool}}\}$ as in Algorithm~\ref{alg:ellipsoidal-minucb},
$\delta_{\mathrm{off}}$, and
$\{\delta_k\}_{k=1}^{K_{\mathrm{ep}}}$ for $\beta_k^{\mathrm{on}}(\delta_k)$, satisfying
\(
\delta_{\mathrm{off}}{+}\sum_{k=1}^{K_{\mathrm{ep}}}\delta_k{\le}\delta_{\mathrm{cert}}
\)
\State Build
$G_{\mathrm{off}}$, $\hat\theta_{\mathrm{off}}$, and
$\beta_{\mathrm{off}}(\delta_{\mathrm{off}})$ from~$D_{\mathrm{off}}$
\State
$L\gets\lceil\log_2 T\rceil$; initialize
$\cH_{1,\ell}\gets\varnothing$ for $\ell=0,1,\dots,L$
\For{each epoch $k=1,2,\dots,K_{\mathrm{ep}}$}
    \State
    $G_k^{\mathrm{on}}\gets I{+}\sum_{s<\tau_k} x_{s,a_s}x_{s,a_s}^{\top}$;\quad
    $\hat\theta_k^{\mathrm{on}}\gets (G_k^{\mathrm{on}})^{-1}\sum_{s<\tau_k} x_{s,a_s}r_s$
    \State
    $\widehat M_k\gets\bigl((G_k^{\mathrm{on}})^{-1}{+}G_{\mathrm{off}}^{-1}\bigr)^{-1}$;\quad
    $\widehat\Delta_k\gets\hat\theta_k^{\mathrm{on}}-\hat\theta_{\mathrm{off}}$
    \State
    $\widehat\rho_k\gets
    \|\widehat\Delta_k\|_{\widehat M_k}
    {+}\beta_k^{\mathrm{on}}(\delta_k)
    {+}\beta_{\mathrm{off}}(\delta_{\mathrm{off}})$
    \For{each $t=\tau_k,\dots,\tau_{k+1}-1$}
        \State Execute the per-round layer loop of
        Algorithm~\ref{alg:ellipsoidal-minucb} at time~$t$,
        using \eqref{eq:epoch-pool-rad}--\eqref{eq:epoch-psi} in place of
        $\mathrm{rad}^{\mathrm{pool}}_{t,\ell}(\cdot)$ when forming the pooled UCB/LCB
    \EndFor
\EndFor
\end{algorithmic}
\end{algorithm}

\begin{theorem}[Regret with epoch-wise learned certificates]
\label{thm:epoch-parallel-regret}
Run Algorithm~\ref{alg:epoch-ell-minucb}.
Let $k(t)$ satisfy
\(
t\in\{\tau_{k(t)},\ldots,\tau_{k(t)+1}-1\}
\)
and define the routed path sum
\[
\widetilde\Psi_T^{\mathrm{ep}}
:=
\sum_{t=1}^T\widehat\rho_{k(t)}\,\widehat\psi_{k(t),t,\ell_t}(x_{t,a_t}).
\]
Then, with probability at least $1-T^{-2}-\delta_{\mathrm{cert}}$,
\[
R_T
\le
\min\left\{
C_{\mathrm{SL}}\sqrt{Td\,L_T^3},
\;
8\sum_{\ell=0}^{\lceil\log_2 T\rceil}
\bigl(\beta_{\mathrm{off}}+\gamma_\ell^{\mathrm{fin}}\bigr)
\sqrt{2|Q_\ell|\,\Lambda_\ell}
+8\,\widetilde\Psi_T^{\mathrm{ep}}
\right\},
\]
where $Q_\ell,\Lambda_\ell,\gamma_\ell^{\mathrm{fin}}$ are as in Theorem~\ref{thm:main}.
\end{theorem}

Theorem~\ref{thm:epoch-doubling-regret} in Appendix~\ref{app:epoch-dd-details} records a common
doubling epoch schedule and closed-form confidence radii under which the routed shift term admits an
additional Cauchy--Schwarz aggregation through~$\mathcal S_{\mathrm{ep}}$.
Proofs of Theorems~\ref{thm:epoch-parallel-cert-valid}, \ref{thm:epoch-parallel-regret}, and
\ref{thm:epoch-doubling-regret} are in Appendix~\ref{app:epoch-learned-proofs}.


==> sections/related_work.tex <==
\section{Related Work}
\label{sec:related}

A broad offline-to-online literature studies how historical data, hints, or source models can
reduce the cost of online learning. Warm-start and transfer approaches combine supervised and bandit
feedback \citep{zhang2019}, use initial hints \citep{cutkosky2022}, handle deficient support in
logged data \citep{tran2021}, and transfer across contextual bandit tasks \citep{cai2024}. Other
work considers weighted hypothesis transfer \citep{bilaj2022}, partially observed confounded
offline data \citep{tennenholtz2020}, offline logs in larger sequential settings
\citep{wagenmaker2023,kausik2024}, and contextual online--offline interaction in pricing
\citep{zhang2025contextualpricing,bu2020icml,bu2024featurepricing}. A related offline contextual
bandit and off-policy learning line learns or evaluates policies from logged feedback under support,
variance, or pessimism constraints \citep{dudik2011,swaminathan2015,wang2024,gabbianelli2024}. These
works establish many ways in which past data can help decision-making, but their main object is not
the online regret value of biased offline evidence after deployment.

The closest comparisons come from two directions. In linear bandits with offline data, prior
observations can lower exploration cost through offline Gram matrices and design-based exploration
when the offline and online parameters coincide \citep{vijayan2025oope}. In multi-armed bandits with
biased offline data, MIN-UCB shows that a learner should exploit offline samples only when the
mismatch is controlled, and otherwise fall back toward online learning \citep{cheung2024}. These two
lines capture the two ingredients we need: coverage in a linear model and safe use of biased offline
information.

What remains open is how to judge offline quality when both ingredients are present in a linear
contextual bandit. Offline coverage alone is not enough because the offline parameter may drift; a
scalar mismatch bound is not enough because actions share features and shift matters by direction.
Our setting therefore asks which feature directions of the offline sample remain reusable online. The
directional certificate is the interface we use to express this quality and to decide when pooled
offline evidence can safely contract online uncertainty.

At the algorithmic level, our online fallback builds on the optimism-based foundations of
contextual and linear bandits: LinUCB and SupLinUCB \citep{li2010,chu2011}, the OFUL analysis
\citep{abbasi2011}, and linear Thompson-style approaches \citep{agrawal2013}. We also relate to
misspecification-robust bandits, where the online reward model may deviate from the assumed linear
class. Classic and follow-up work includes \citet{ghosh2017} and \citet{takemura2021}; more recent
developments include \citet{foster2020misspec} and \citet{krishnamurthy2021}. Here the online model
remains linear; the difficulty is that the \emph{offline} parameter may differ from the online one in
a structured, direction-dependent way. Our contribution is to encode that mismatch through a
directional certificate and use it inside a hybrid pooled/online optimistic rule.


==> shared/macros/experiment_macros_generated.tex <==
% Auto-generated by experiments.py (run main or --extended).
\makeatletter
\gdef\ExtNoOracleCertValid{yes}
\gdef\ExtDiagLinFinal{$203.6 \pm 6.1$}
\gdef\ExtDiagEllipFinal{$202.4 \pm 6.0$}
\gdef\ExtDiagRidgeFinal{$107.2 \pm 7.4$}
\gdef\ExtDiagTEllip{$0.78$}
\gdef\ExtDiagTRidge{$52.48$}
\gdef\ExtCorrLinFinal{$65.3 \pm 17.7$}
\gdef\ExtCorrRidgeFinal{$37.1 \pm 5.4$}
\gdef\ExtCorrEllipOFinal{$47.6 \pm 9.5$}
\gdef\ExtCorrEllipIsoFinal{$47.6 \pm 9.5$}
\gdef\ExtCorrEllipNFinal{$56.3 \pm 15.4$}
\gdef\ExtCorrGreedyFinal{$71.6 \pm 4.0$}
\gdef\ExtCorrTEllipVsLin{$5.00$}
\gdef\ExtCorrTEllipVsRidge{$-6.49$}
\gdef\ExtCorrTEllipVsIso{$0.00$}
\gdef\ExtCorrTEllipNVsLin{$2.17$}
\gdef\ExtCorrTRidgeVsLin{$7.88$}
\makeatother


==> shared/macros/paper_macros_generated.tex <==
% Auto-generated by experiments.py --paper
% PaperImp* = oracle-geometry ellipsoid; PaperNoOracle* = certificate_no_oracle
\gdef\PaperImpFiveHundredMean{36.5}
\gdef\PaperImpFiveHundredCI{1.7}
\gdef\PaperImpFinalMean{1.0}
\gdef\PaperImpFinalCI{1.5}
\gdef\PaperIsoImpFiveHundredMean{39.6}
\gdef\PaperIsoImpFiveHundredCI{1.5}
\gdef\PaperIsoImpFinalMean{0.2}
\gdef\PaperIsoImpFinalCI{1.1}
\gdef\PaperNoOracleImpFiveHundredMean{0.7}
\gdef\PaperNoOracleImpFiveHundredCI{2.0}
\gdef\PaperNoOracleImpFinalMean{1.2}
\gdef\PaperNoOracleImpFinalCI{1.6}
\gdef\PaperBundleNRuns{36}


==> style/experiment_macros.tex <==
\makeatletter
\gdef\ExtNoOracleBiasBoundValid{yes}
\gdef\ExtDiagLinFinal{$203.6 \pm 6.1$}
\gdef\ExtDiagEllipFinal{$202.4 \pm 6.0$}
\gdef\ExtDiagRidgeFinal{$107.2 \pm 7.4$}
\gdef\ExtDiagTEllip{$0.78$}
\gdef\ExtDiagTRidge{$52.48$}
\gdef\ExtCorrLinFinal{$65.3 \pm 17.7$}
\gdef\ExtCorrRidgeFinal{$37.1 \pm 5.4$}
\gdef\ExtCorrEllipOFinal{$47.6 \pm 9.5$}
\gdef\ExtCorrEllipIsoFinal{$47.6 \pm 9.5$}
\gdef\ExtCorrEllipNFinal{$56.3 \pm 15.4$}
\gdef\ExtCorrGreedyFinal{$71.6 \pm 4.0$}
\gdef\ExtCorrTEllipVsLin{$5.00$}
\gdef\ExtCorrTEllipVsRidge{$-6.49$}
\gdef\ExtCorrTEllipVsIso{$0.00$}
\gdef\ExtCorrTEllipNVsLin{$2.17$}
\gdef\ExtCorrTRidgeVsLin{$7.88$}
\makeatother

